FORTRESS II: FORTRAN programs for solving coupled Gross-Pitaevskii equations for spin-orbit coupled spin-2 Bose-Einstein condensate

We provide here a set of three OpenMP parallelized FORTRAN 90/95 programs to compute the ground states and the dynamics of trapped spin-2 Bose-Einstein condensates (BECs) with anisotropic spin-orbit (SO) coupling by solving a set of five coupled Gross-Pitaevskii equations using a time-splitting Fourier spectral method. Depending on the nature of the problem, without any loss of generality, we have employed the Cartesian grid spanning either three-, two-, or one-dimensional space for numerical discretization. To illustrate the veracity of the package, wherever feasible, we have compared the numerical ground state solutions of the full mean-field model with those from the simplified scalar models. The two set of results show excellent agreement, in particular, through the equilibrium density profiles, energies and chemical potentials of the ground-states. We have also presented test results for OpenMP performance parameters like speedup and the efficiency of the three codes.

==> FORTRESS-II/README <==
===============================================================================
FORTRESS-II consists of a set of three FORTRAN 90/95 codes with OpenMP 
parallelization and can be used to solve coupled Gross-Pitaevskii equations
for a spin-orbit coupled spin-2 Bose-Einstein condensate. The codes are
apt to study the static properties like computing the ground state energy, 
density profiles, chemical potentials, and rms sizes, etc, as well
as the real-time dynamics.
===============================================================================
 
What you need to have on your system to use these codes?

The codes use FFTW software library which is freely available
on http://www.fftw.org/. The software library needs to be installed
on the system if not already installed. Please refer to
http://www.fftw.org/fftw2_doc/fftw_6.html for the installation 
instructions. Please take note that while configuring FFTW suitable 
flags (--with-openmp --enable-threads) need to be invoked to enable
FFTW threading.

The system should have a FORTRAN compiler installed on it.
It can be any of freely available FORTRAN compilers
like GNU's gfortran, Fortran 95 compiler f95, or to have a better
performance it can be Intel's FORTRAN compiler. Testing of the
codes has been done with all these three compilers.

It is advisable to unlimit the stack size on your machine too,
especially while using 2D and 3D codes with large array sizes.
On bash, sh or ksh shells this can be done by using
ulimit -s unlimited; not doing so may cause the segmentation
fault. And also increase the OpenMP stack size by 
executing at the command prompt-  export OMP_STACKSIZE=1024M (to
set it to say 1024MB)

-------------------------------------------------------------------------------
-------------------------------------------------------------------------------
Installation of the FORTRESS:

Unzip the FORTRESS-II.zip in the directory of your choice using
unzip FORTRESS-II.zip

This will create a single FORTRESS-II folder in user's current directory.
-------------------------------------------------------------------------------
-------------------------------------------------------------------------------
The FORTRESS-II folder consists of three subfolders:
(1) SOURCE_FILES (2) INPUT (3) OUTPUT


./FORTRESS-II/SOURCE_FILES has the three codes of this package, namely
(a) imretime1D_spin2.f90
(b) imretime2D_spin2.f90
(c) imretime3D_spin2.f90


'imretime3D_spin2.f90' can be used to solve coupled
GP equations 1(a)-1(c) in imaginary or realtime in 3D. Similarly
'imretime2D_spin2.f90' can be used to solve these equations
for q2D and 'imretime1D_spin2.f90' can be used to solve 
these equations for q1D BEC.


(2) ./FORTRESS-II/INPUT has three folders within it: 1D, 2D, 3D.
    In the realtime simulation the necessary input data files
    should be in these sub-subfolders for 1D, 2D and 3D realtime 
    simulations.

(3) Similarly, ./FORTRESS-II/OUTPUT has three folders within it, namely 
    1D, 2D, 3D. The output files for the 1D, 2D and 3D codes are,
    respectively written in these sub-subfolders.
-------------------------------------------------------------------------------
-------------------------------------------------------------------------------
Before you compile the code:

Please take note that SWITCH_IM = 1 or 0 for imaginary time and 
realtime propagations, respectively. When SWITCH_IM = 0 the code would be needing
an initial solution written in file './FORTRESS-II/INPUT/*D/initial_sol.dat'
where *=1, 2, 3 for 1D, 2D, 3D codes, respectively.
The contents of this file need to be in the same pattern
as that of solution_file_*.dat described below. When SWITCH_IM = 1
magnetization value between 0<=M<2 need to be entered at command
line prompt by the user.

OPTION_FPC = 1, 2 or 3 for directing the code to choose the 
initial guess suitable for ferromagnetic, antiferromagnetic 
or cyclic interactions, respectively; in case Gaussian initial
guess has to be selected then OPTION_FPC = 4. 

SWITCH_SOC = 0 if GAMMAX = GAMMAY = GAMMAZ = 0, otherwise
SWITCH_SOC = 1 if any of GAMMAX, GAMMAY, GAMMAZ is non-zero

For more details, please read 'README_INPUT' in the 'INPUT'
folder of the package.
-------------------------------------------------------------------------------
-------------------------------------------------------------------------------
How to compile the codes?

With GNU Fortran compiler: 
(a) For compiling without OpenMP execute: gfortran imretime1D_spin2.f90 -I/usr/local/include/ -lfftw3 -lfftw3_threads -lpthread -lm -llapack -lblas
(b) For compiling with OpenMP execute: 
    (1) gfortran imretime1D_spin2.f90 -I/usr/local/include/ -lfftw3_omp -lfftw3 -fopenmp \ 
        -m64 -I${MKLROOT}/include -Wl,--no-as-needed -L${MKLROOT}/lib/intel64 \ 
        -lmkl_gf_lp64 -lmkl_core -lmkl_gnu_thread -lpthread -lm -ldl
    (2) gfortran imretime1D_spin2.f90 -I/usr/local/include/ -lfftw3_omp -lfftw3 -lm -fopenmp \ 
       ./INCLUDE/libtmglib.a ./INCLUDE/liblapack.a ./INCLUDE/librefblas.a
    (3) gfortran imretime1D_spin2.f90 -I/usr/local/include/ -lfftw3_omp -lfftw3 -lm -fopenmp -llapack -lblas

    Please take note that /usr/local/include/ is the location of the file FFTW-software-library provided the file 'fftw3.f03' 
    that defines Fortran 2003 interfaces for all of its C routines. If this file 'fftw3.f03' is present in different folder, then
    the corresponding path needs to be provided. 
    

    
With Intel® Fortran Compiler
(a) For compiling without OpenMP execute: ifort imretime1D_spin1.f90 -lfftw3 -lfftw3_threads -lpthread -lm -mkl=sequential
(b) For compiling with OpenMP execute: 
    (1) ifort imretime1D_spin2.f90 -lfftw3_omp -lfftw3 -lm -qopenmp -mkl=parallel
    (2) ifort imretime1D_spin2.f90 -lfftw3_omp -lfftw3 -lm -qopenmp ./INCLUDE/libtmglib.a ./INCLUDE/liblapack.a ./INCLUDE/librefblas.a
    (3) ifort imretime1D_spin2.f90 -lfftw3_omp -lfftw3 -lm -qopenmp -llapack -lblas

With f95 fortran compiler
(a) For compiling without OpenMP execute: f95 imretime_spin1_1D.f90 -lfftw3 -lfftw3_threads -lpthread -lm -llapack -lblas
(b) For compiling with OpenMP execute: 
    (1) f95 imretime1D_spin2.f90 -I/usr/local/include/ -lfftw3_omp -lfftw3 -fopenmp \ 
        -m64 -I${MKLROOT}/include  -Wl,--no-as-needed -L${MKLROOT}/lib/intel64 \ 
        -lmkl_gf_lp64 -lmkl_core -lmkl_gnu_thread -lpthread -lm -ldl
    (2) f95 imretime1D_spin2.f90 -I/usr/local/include/ -lfftw3_omp -lfftw3 -lm -fopenmp \ 
       ./INCLUDE/libtmglib.a ./INCLUDE/liblapack.a ./INCLUDE/librefblas.a
    (3) f95 imretime1D_spin2.f90 -I/usr/local/include/ -lfftw3_omp -lfftw3 -lm -fopenmp -llapack -lblas

For serial execution of the code: Set OPENMP_THREADS = FFTW_THREADS = 1 in the BASIC_DATA module

    For compilation option (1) Intel's Math Kernal Library needs to be 
    installed on the system if not already installed with intel's compiler. For installation
    instructions please refer to
    https://software.intel.com/content/www/us/en/develop/tools/math-kernel-library.html.

    For compilation option (2), LAPACK software package needs to be installed on the system.
    For installation instuctions, please refer to http://www.netlib.org/lapack/. For this
    compilation option, ./INCLUDE/ is the location of LAPACK libraries libtmglib.a, liblapack.a,
    librefblas.a. and can be replaced by the location of these libraries on the user's machine.

    To compile with option (3), one needs to install lapack and blas libraries, e.g. using
    sudo apt-get install libblas3 liblapack3 libblas-dev liblapack-dev (on ubuntu) 

    Please take note that the best performance can be obtained with compilation 
    option (1), whereas the compilation option (3) is the slowest one.
    For compilation option (2), ./INCLUDE/ needs to be replaced by the location of LAPACK libraries
    libtmglib.a, liblapack.a, and librefblas.a on the user's machine.

Note: For compilation with OpenMP or auto-parallelization it is advisable to 
      unlimit the shell stack size limit by executing at the command prompt-  ulimit -s unlimited            
      And increase the OpenMP stack size to sufficiently large value by executing at the command 
      prompt-  export OMP_STACKSIZE=1024M 

The OpenMP and FFTW threads should be judiciously chosen
as per the available computational resources and array sizes
of the wave functions.
-------------------------------------------------------------------------------
-------------------------------------------------------------------------------
Where are the output file written?

The various output files are written in ./FORTRESS-II/OUTPUT/1D,
./FORTRESS-II/OUTPUT/2D, and  ./FORTRESS-II/OUTPUT/3D for 1D, 2D and 3D
simulations, respectively.
-------------------------------------------------------------------------------
-------------------------------------------------------------------------------
What is in the output files:

Description of contents of "file1_*.dat"

The contents of "file1_*.dat" (where '*' is 'im' or 're') are described in
section 5 of the preprint (please refer to this section for details).
Basically this file will list 
(a) all the input parameters set during the run of the code 
(b) total norm, energy, chemical potentials of the component wave-functions,
absolute values of component wave-functions at the origin, and
magnetization corresponding to initial guess/solution, for the transient
solution obtained after NSTP time iterations, energy, rms sizes obtained 
after STP time iterations and for the converged
solution (this third entry in real-time code will simply correspond
to the solution after NITER iterations).
-------------------------------------------------------------------------------

-------------------------------------------------------------------------------
Description of contents of "file2_*.dat"

In this file, data would be written after every STP iterations.
Contents-
1st column: Time 
2nd column: Energy
3th column: rms size of 1st component
4th column: rms size of 2nd component
5th column: rms size of 3rd component
6th column: rms size of 4th component
7th column: rms size of 5th component
-------------------------------------------------------------------------------

-------------------------------------------------------------------------------
Description of contents of "file3_*.dat"

In this file, data would be written after every STP iterations.
Contents-
1st column: Time
2nd column: Norm of 1st component
3th column: Norm of 2nd component
4th column: Norm of 3rd component
5th column: Norm of 4th component
6th column: Norm of 5th component
7th column: sum of norms of individual component
8th column: Magnetization
------------------------------------------------------------------------------

-------------------------------------------------------------------------------
Description of contents of "tmp_solution_file.dat"

In this file, transient solutions would be written after every NSTP iterations.
Contents-

For 1D-
1st column : x
2nd column : density of 1st component
3rd column : phase of 1st component
4th column : density of 2nd component
5th column : phase of 2nd component
6th column : density of 3rd component
7th column : phase of 3rd component
8th column : density of 4th component
9th column : phase of 4th component
10th column: density of 5th component
11th column: phase of 5th component

For 2D-
1st column : x
2nd column : y
3rd column : density of 1st component
4th column : phase of 1st component
5th column : density of 2nd component
6th column : phase of 2nd component
7th column : density of 3rd component
8th column : phase of 3rd component
9th column : density of 4th component
10th column: phase of 4th component
11th column: density of 5th component
12th column: phase of 5th component


For 3D-
1st column : density of 1st component
2nd column : phase of 1st component
3rd column : density of 2nd component
4th column : phase of 2nd component
5th column : density of 3rd component
6th column : phase of 3rd component
7th column : density of 4th component
8th column : phase of 4th component
9th column : density of 5th component
10th column: phase of 5th component
-------------------------------------------------------------------------------

-------------------------------------------------------------------------------
Description of the contents of "convergence.dat"

This file is written in only imaginary time propagation, i.e. when SWITCH_IM = 1.
Contents-
1st column: time
2nd column: convergence parameter
-------------------------------------------------------------------------------

-------------------------------------------------------------------------------
Description of "solution_file_*.dat"

In this file, final converged solution is written in case SWITCH_IM = 1 
or solution after NITER is written in case SWITCH_IM = 0
Contents-

For 1D-
1st column : x
2nd column : density of 1st component
3rd column : phase of 1st component
4th column : density of 2nd component
5th column : phase of 2nd component
6th column : density of 3rd component
7th column : phase of 3rd component
8th column : density of 4th component
9th column : phase of 4th component
10th column: density of 5th component
11th column: phase of 5th component

For 2D-
1st column : x
2nd column : y
3rd column : density of 1st component
4th column : phase of 1st component
5th column : density of 2nd component
6th column : phase of 2nd component
7th column : density of 3rd component
8th column : phase of 3rd component
9th column : density of 4th component
10th column: phase of 4th component
11th column: density of 5th component
12th column: phase of 5th component

For 3D-
1st column : density of 1st component
2nd column : phase of 1st component
3rd column : density of 2nd component
4th column : phase of 2nd component
5th column : density of 3rd component
6th column : phase of 3rd component
7th column : density of 4th component
8th column : phase of 4th component
9th column : density of 5th component
10th column: phase of 5th component
===============================================================================

NOTE :  With this submission, in ./FORTRESS-II/OUTPUT/1D,./FORTRESS-II/OUTPUT/2D, 
        and  ./FORTRESS-II/OUTPUT/3D for 1D, 2D and 3D simulations, respectively, 
        we are providing only the contents of file1_im.dat for the current 
        set of parameters in the codes and file1_re.dat for 1D real-time 
        simulation.
       
        The test input files initial_sol.dat needed for real-time simulations
        are in the ./FORTRESS-II/INPUT/1D and ./FORTRESS-II/INPUT/2D for 1D and 2D 
        simulations, respectively. 


